Galaxy-galaxy lensing estimators and their covariance properties

We study the covariance properties of real space correlation function estimators -- primarily galaxy-shear correlations, or galaxy-galaxy lensing -- using SDSS data for both shear catalogs and lenses (specifically the BOSS LOWZ sample). Using mock catalogs of lenses and sources, we disentangle the various contributions to the covariance matrix and compare them with a simple analytical model. We show that not subtracting the lensing measurement around random points from the measurement around the lens sample is equivalent to performing the measurement using the lens density field instead of the lens over-density field. While the measurement using the lens density field is unbiased (in the absence of systematics), its error is significantly larger due to an additional term in the covariance. Therefore, this subtraction should be performed regardless of its beneficial effects on systematics. Comparing the error estimates from data and mocks for estimators that involve the over-density, we find that the errors are dominated by the shape noise and lens clustering, that empirically estimated covariances (jackknife and standard deviation across mocks) are consistent with theoretical estimates, and that both the connected parts of the 4-point function and the super-sample covariance can be neglected for the current levels of noise. While the trade-off between different terms in the covariance depends on the survey configuration (area, source number density), the diagnostics that we use in this work should be useful for future works to test their empirically-determined covariances.

==> referee_report <==
>The paper "Galaxy-galaxy lensing estimators and their covariance
>properties." by Singh et al. deals with different estimators of
>galaxy-galaxy lensing used in the literature. There has been a debate
>about whether the signal around random points should be subtracted
>from the signal around real lenses. This paper provides very
>interesting additional reasons for doing so, making an argument
>similar to the one by Landy & Szalay (1993) about clustering
>measurements. Hence, this paper should be published in MNRAS after
>some moderate revision.

We thank the Referee for providing a constructive report that helped 
in improving the quality of the paper. We respond to Referee’s comments
below. Any changes in the paper are highlighted in ‘cyan’ color.

>My main points are:

>The presentation could be improved by more clearly distinguishing
>between the randomly rotated mock sources and the QPM mock
>lenses. Maybe it would be useful not to use the word 'mock' for
>both.

We have changed the wording. "mocks sources" has been replaced by
"rotated sources"

>The introduction of the source catalogue is very brief. While I
>don't think that shape measurement biases or photo-z systematics
>really matter for this study, it would be adequate to add a sentence
>or two about how those were determined/corrected.

We have added discussion in section 3.3.

>  It is not mentioned how big the jackknife regions are. Given there
>  are 100 regions over the SDSS footprint I guess each patch is about
>  150deg^2 with a side length >100Mpc at the lens redshift. But I
>  think it would be good to quantify these things in the text.

We have added the numbers in section 2.4.

>  Sect.4.1 and following: The "spurious systematic signal at large
>  scales" is mentioned over and over again. Add a couple of sentences
>  about the possible causes of this signal. Just referring to
>  Mandelbaum et al. (2005, 2013) isn't sufficient for such an
>  important piece of information.

We have added a brief discussion in the text of section 4.1.

> Sect.4.2: Explain in a few words why the effective window function
>  of 'Std' is so much larger than the one for jackknife.

We have added a brief statement.

> Sect.4.3.2: I'm not sure I understand the statement "possibly due to
>  low-level clustering in the random catalogs as they match the
>  selection function of LOWZ". Are you talking about the angular
>  selection function here? Why would that lead to a signal?

Because the random lens samples account for the small incompleteness in the angular selection
function, they are not actually distributed in a completely random way.  
This leads to a small but nonzero P_{gg}-like term in the
randoms which then contributes to the covariance. The covariance is 
(N_g+P_{gg})(P_{\gamma\gamma}+N_\gamma)

> Sect.4.5 stands a bit separate. I guess the motivation of this
>  section is to show that jackknife or subsampling errors are fine if
>  the Delta_Sigma_gR estimator is used. The motivation for this
>  section should be made clear at the beginning.

We have added a brief statement of the motivation for this section at the start of section 4.5.

> The language needs to be improved. Many articles are missing, and
>  the manuscript would benefit from proof-reading by a native speaker
>  (perhaps one of the co-authors?). In particular, Sect.2 struck me as
>  being slightly inferior in language.

The entire manuscript has now been proof-read by a native English speaker.

>Minor points:

> Sect.1: When talking about the study by Shirasaki et al. (2016) note
>  that also Blake et al. (2016) compared GGL covariance matrices
>  estimated with different methods.

We have cited Blake et al. 2016 paper in the introduction also. Based
on our private communication with the lead author Chris Blake, the
randoms subtraction was not performed when computing covariances with mock catalogs in
that work (even though it was performed in the real data).

> Eq.5: Define P_delta,delta.
Done.

> Eq.6: Define Sigma_Rs not only Sigma_ls.
Done.

> Sect.2.3: When you say "from our sample" refer to the section where
>  the sample is described or maybe even add that this is the BOSS-LOWZ
>  sample.

Changed to clarify that this estimation is done empirically when measuring the signal.

> Sect.3.3: I would change the title of this subsection to
>  "Re-Gaussianisation shapes and photo-z".
Changed

> Fig.5: Did you mix up the labels for the green and yellow lines?
Yes.  Fixed.

----------------------------------------------------
Other changes

- We have made major changes in the derivation for covariance for
  projected correlation functions, have introduced a new appendix
  A2, and also made changes in the appendix for the galaxy-galaxy lensing case
  (appendix A3 in current version). 
  In the previous version, we assumed that integration length \Pi 
  is long and carried out the integrals \int d\Pi e^{ik_parallel\Pi} to get
  delta_D(k_\parallel). Then the normalization was set to the area at
  the effective redshift of the sample. 
  In the current version, we make the simplifying assumption
  $P(k)~P(k_perp)$, and then carry out integration over
  k_parallel. The main difference is that in the current version we
  get an additional factor ~\Delta\Pi/L_W, which was effectively set to 1
  in the previous version. As a result, in the previous version, we
  underestimated the cosmic variance terms in the case of galaxy-lensing cross correlations
  (\Delta\Pi/L_W~1.4) and overestimated them in the case of galaxy
  clustering (\Delta\Pi/L_W~0.4). Since the cosmic variance term contributes
  <~10% at all scales, our results for galaxy-lensing change by <~4% at
  all scales.

- Abstract: Corrected ambiguous language.

- Eq. A17: Corrected a typo in a few of the subscripts.

- We have also made minor changes when citing the Shirasaki et al. 2016
  paper, to reflect the substantial changes in conclusions in the updated version of that paper.

